Evaluating the Effects of Digital Privacy Regulations on User Trust

In today's digital society, issues related to digital privacy have become increasingly important. Issues such as data breaches result in misuse of data, financial loss, and cyberbullying, which leads to less user trust in digital services. This research investigates the impact of digital privacy laws on user trust by comparing the regulations in the Netherlands, Ghana, and Malaysia. The study employs a comparative case study method, involving interviews with digital privacy law experts, IT educators, and consumers from each country. The main findings reveal that while the General Data Protection Regulation (GDPR) in the Netherlands is strict, its practical impact is limited by enforcement challenges. In Ghana, the Data Protection Act is underutilized due to low public awareness and insufficient enforcement, leading to reliance on personal protective measures. In Malaysia, trust in digital services is largely dependent on the security practices of individual platforms rather than the Personal Data Protection Act. The study highlights the importance of public awareness, effective enforcement, and cultural considerations in shaping the effectiveness of digital privacy laws. Based on these insights, a recommendation framework is proposed to enhance digital privacy practices, also aiming to provide valuable guidance for policymakers, businesses, and citizens in navigating the challenges of digitalization.

==> project_card.tex <==
% \section*{The Project Card}
% % \begin{enumerate}
% %     \item Research question(s)
% %     \item Approach, emphasis on methods
% %     \item Main results and contribution(s)
% % \end{enumerate}

% \begin{framed}

% Research question(s):
% \begin{description}
%     \item[RQ1] 
% \end{description}
% \end{framed}

% \begin{framed}
% Research method(s):
% \begin{description}
%     \item[M1] 
% \end{description}

% % Research approach:
% % \begin{description}
% %     \item[A1]  \\
    
% %     \item[A2]  \\
    
% %     \item[A3] To address {\bf RQ1} we use methodology M1 and develop an instrument that can statistically compare the operations of a cluster across different time periods.
% % \end{description}
    
% \end{framed}

% \newpage
% Main results and contribution:
% \begin{framed}
% \begin{description}

%     \item[R1]  

%     \item[C1]  
    
% \end{description}
% \end{framed}

